MgNO: Efficient Parameterization of Linear Operators via Multigrid

In this work, we propose a concise neural operator architecture for operator learning. Drawing an analogy with a conventional fully connected neural network, we define the neural operator as follows: the output of the $i$-th neuron in a nonlinear operator layer is defined by $O_i(u) = \sigma\left( \sum_j W_{ij} u + B_{ij}\right)$. Here, $ W_{ij}$ denotes the bounded linear operator connecting $j$-th input neuron to $i$-th output neuron, and the bias $ B_{ij}$ takes the form of a function rather than a scalar. Given its new universal approximation property, the efficient parameterization of the bounded linear operators between two neurons (Banach spaces) plays a critical role. As a result, we introduce MgNO, utilizing multigrid structures to parameterize these linear operators between neurons. This approach offers both mathematical rigor and practical expressivity. Additionally, MgNO obviates the need for conventional lifting and projecting operators typically required in previous neural operators. Moreover, it seamlessly accommodates diverse boundary conditions. Our empirical observations reveal that MgNO exhibits superior ease of training compared to other CNN-based models, while also displaying a reduced susceptibility to overfitting when contrasted with spectral-type neural operators. We demonstrate the efficiency and accuracy of our method with consistently state-of-the-art performance on different types of partial differential equations (PDEs).

==> Archive.tex <==
\paragraph{Skip connection}

\subsection{Multigrid based non local convolution operator}
{\color{red} put some detailed discriptions about MgNet}

Here, we give a brief introduction to some key components of a V-cycle multigrid in the convolutional language as an operator form $f$ to $u$:
\begin{enumerate}
    \item \textbf{Input ($f$) and Initialization}: \( f^1 = f \), along with an initial guess, \( u^{1,0} = 0 \).
    \item \textbf{Iteration (Smoothing) Process}: The algorithm refines \( u \) iteratively using the relation:
    \begin{equation}\label{eq:smoothing}
    u^{\ell,i} = u^{\ell,i-1} + B^{\ell,i} \ast \left(f^{\ell}- A^\ell \ast u^{\ell,i-1}\right)
    \end{equation}
    for $\ell=1:J$ and \( i\leq \nu_\ell \). The iteration closely mirrors the Jacobian method, with the iterated solution \( u^{\ell,i} \) acting as the extracted feature. 
    \item \textbf{Hierarchical Structure by Restriction and Prolongation}: 
    The superscript \( \ell \) signifies the specific level or phase within the hierarchical, multigrid structure. 
    In particular, we from the residual  restrict the input $f^{\ell}$ and current $u^{\ell}$ to the coarser level by  convolution with stride 2 via \begin{equation}
          f^{\ell+1}= R_{\ell}^{\ell+1}\ast_2\left(f^{\ell}-A^{\ell} \ast u^{\ell}\right) \in \mathbb{R}^{d_{\ell+1}\times d_{\ell+1} \times n} \text{ and } 
          u^{\ell+1,0}= 0
    \end{equation}and then do the smoothing iteration as in ~\eqref{eq:smoothing} to obtain the correction from coarse level. Then, we prolong the correction from the coarse level to the fine level by a de-convolutional with stride 2 (the transpose of the restriction operation).  After prolongation to a coarser level, one can either choose to further prolong to an even coarser level (termed as the Backslash-cycle) or opt for post-smoothing followed by prolongation (known as the V-cycle).
\end{enumerate}


However, the complexity issue rises if we just simply parameterize each $\mathcal W^\ell_{ij}$ operator as $\mathcal W_{Mg}$ with multi-channel. 
If that, the total number of parameters for $\mathcal W^\ell_{ij}$ equals $\mathcal O\left(\log(d) \widetilde n^2\right)$, where $\widetilde n$ is the number of channels in each $\mathcal W_{Mg}$. 
As a trade-off between expressivity and complexity, we propose sharing the inner channels in teach $\mathcal W^\ell_{ij}$ for different $i,j$ and fixing the number of channels to be $n$ as the same number of neurons. Practically, we can implement this $\mathcal W_{Mg}$ as a multi-channel V-cycle multigrid method. Consequently, the total number of parameters in $\mathcal W^\ell = \mathcal W_{Mg}$ is reduced to . 

For the nonlinear activation operator, there exist $\sigma:\mathbb R \mapsto \mathbb R$ and two non-zero eigenfunctions $\bm y_{\sigma}, \bm y'_{\sigma}  \in \mathcal Y$ such that 
    \begin{equation}
        \bm \sigma\left(a \bm y_{\sigma}\right) = \sigma(a)\bm y'_{\sigma} \quad \forall a \in \mathbb R.
    \end{equation}

\begin{remark}In previous work about operator learning, the nonlinear activation functions are all defined point-wise. 
Given that $\mathcal X$ and $\mathcal Y$ are all functions on $\Omega \subset \mathbb R^d$, the point-wise activation operator ${\bm \sigma}$ is defined as
        \begin{equation}
            \bm \sigma(u)(x) = \sigma \circ u(x),
        \end{equation}
        where $\sigma: \mathbb R \mapsto \mathbb R$ is the classical activation function in standard neural networks.

It is easy to see that the point-wise defined activation operator satisfies the previous assumption by taking
\begin{equation}
    \bm y_{\sigma} = \bm y'_{\sigma} = \bm 1(x),
\end{equation}
where $\bm 1(x) \in \mathcal Y$ is the constant function on $\Omega$.
\end{remark}


\paragraph{MgIter}

The operator MgIter processes a multichannel input feature, denoted as $\vf^{\ell}$, in conjunction with an initial guess, represented by $\vu^{\ell,0}$. This initial guess is initialized to zero at the commencement of the linear operator $\mathcal W_{ij}$. As part of the process, the operator iterates on $\vu$ using the relation:
\[ \vu^{\ell,i} = \vu^{\ell,i-1} + \tB\ast \left(f^{\ell}-\tA\ast \vu^{\ell,i-1}\right) \]
for \( i\leq \nu_\ell \), where this resides in the space \(\mathbb{R}^{d_\ell\times d_\ell \times c}\).

The superscript $\ell$ signifies a particular level or phase within a hierarchical structure. It is worth noting that this iteration closely resembles the Jacobian method applied to solve the linear equation $\tA \ast \vu = \vf$. Consequently, the iterated solution $\vu^{\ell,i}$ serves as the extracted feature. This extraction mechanism is governed by the learnable convolutions, $\tA$ and $\tB$, which ultimately define the physical properties that these features adhere to.

Many intricate nonlinear operators can be distilled into solving a sequence of the equation type $\tA \ast \vu = \vf$. In practical scenarios, the parameters $\tA$ and $\tB$ exhibit variations across levels and iterations.

Furthermore, the channel count, denoted as $c$, remains consistent between the initial state $\vu^{\ell, 0}$ and the resultant feature $\vu^{\ell,i}$. Lastly, the iteration count, represented by $\nu_\ell$, functions as a hyperparameter and remains invariant across all levels.




\paragraph{Restriction}
The multigrid idea is to perform the iteration on multiple grids so that the high frequency components are smoothed out and the low frequency components are preserved. In the context of operator learning, the coarse gird iteration extend the convolution range and The operator \textsc{restriction} takes the feature $\vu^{\ell}$ on the fine grid and restricts it to the coarse grid by $\vu^{\ell+1,0}= \Pi^{\ell+1}_{\ell}\ast_2\vu^{\ell} \in \mathbb{R}^{d_{\ell+1}\times d_{\ell+1} \times c}$. The restriction operator $\Pi^{\ell+1}_{\ell}$ is a learnable convolution with stride 2. The number of channels $c$ is the same as the input feature $\vu^{\ell}$ and the output feature $\vu^{\ell+1,0}$.
\paragraph{Relation with UNet and other neural operators}
Our network resemble the UNet architecture. However, there are several differences between our network and UNet. First of all, our network is a linear operator between neurons and it serves as one layer of the whole neural operator. u and f
\paragraph{Argument incorporated with boudary conditions \& expressivity}


\section{Method}

% Herein, we first introduce the basic architecture of the general nonlocal neural operators \citep{li2020neural,li2020multipole,li2020fourier,you2022nonlocal,you2022learning}, which are comprised of three building blocks. 

% First, the input function, $\vg(\vx)$, is lifted to a higher-dimensional (actually, that is the number of neurons in the first hidden layer) representation via 
% \begin{equation}
% \vh^0(\vx)=\mathcal{P}\circ \vg(\vx):=P[\vg(\vx)]^T+\vb,
% \end{equation}
% where $P\in\mathbb R^{d_g\times d_h}$ and $\vb\in\mathbb R^{d_h}$ are trainable parameters which define an affine pointwise mapping. 

% Then, the feature vector function $\vh^0(\vx)$ goes through an iterative layer block, where the layer update is defined via the sum of a local linear operator, a nonlocal integral kernel operator, and a bias function:
% $$\vh^{l+1}(\vx)=\mathcal{F}^{l+1}[\vh^l](\vx).$$
% Here, $\sigma$ is the activation function. $\mathcal{F}^1,\cdots,\mathcal{F}^{L}$ are the nonlinear operator layers defined as
% \begin{equation}
% \mathcal{F}[\vh](\vx):=\sigma(W\vh(\vx)+\vc+\mathcal{A}[\vh](\vx))
% \end{equation}
% where $W\in\mathbb R^{d_h\times d_h}$ and $\vc\in\mathbb R^{d_h}$ are learnable tensors and $\mathcal{A}$ is a linear nonlocal operator defined as:
% \begin{equation}
% \mathcal{A}[\vh](\vx):=\int_{\Omega} \kappa(\vx,\vy)\vh(\vy) d\vy.
% \end{equation}
% $\Omega$ can be taken either as the whole computational domain, or a neighborhood of $\vx$. In the later case, we often take it as $B_{\delta}(\vx)$, a ball of radius $\delta$ centered at $\vx$. \blue{Here, the definition of $\mathcal A$ is not clear regarding the operations in channels. Consider the following definition via neurons
% \begin{equation}
%     \left[ \mathcal A_{ij} h_j\right] \in \mathcal Y, \quad \forall i=1:d_h
% \end{equation}
% and 
% \begin{equation}
%     \mathcal A_{ij} \in \mathcal L(\mathcal Y, \mathcal Y_j \in \mathcal Y, \quad i,j = d_h.
% \end{equation}
% }

% Finally, the output $\vu(\vx)$ is obtained via a projection layer by mapping the last hidden layer representation $\vh^L(\vx)$ as:
% $$\vu(\vx)=\mathcal{Q}\circ \vh^L(\vx)$$
% where the pointwise function $\mathcal{Q}$ is often taken as a dense neural network of 2 layers from $\mathbb R^{d_h} \mapsto \mathbb R$, i.e.,
% $$\mathcal{Q}(\vx):=Q_2\sigma(Q_1\vx+\vq_1)+\vq_2$$
% where $Q_1$, $Q_2$, $\vq_1$ and $\vq_2$ are the appropriately sized matrices and vectors that are part of the learnable parameter set, and $\sigma$ is an activation function (e.g., ReLU).


As defined before, we need to find 
$\mathcal W_{ij}^\ell \in \mathcal L\left(\mathcal Y, \mathcal Y\right), \quad i=1:n_{\ell-1}, j=1:n_\ell.$
However, practically and numerically, we have to parameterize $\mathcal W_{i,j}$ in some finite-dimensional spaces. For example, General Neural Operator parametrizes $\mathcal W^\ell_{i,j}$ as $(\mathcal W^\ell_{i,j} u)(x) = \int \mathcal K_{ij}(x,y)u(y)dy.$
Therefore, General Neural Operator changes the problem to how to parameterize the kernel $\mathcal K_{ij}(x,y)$ between different neurons.
In practice, both $\mathcal X$ and $\mathcal Y$ are essentially finite-dimensional function spaces. However, even if they are finite-dimensional function spaces, it may still be very hard to parametrize $\mathcal W_{i,j}^\ell$ efficiently.
For example, in most cases, $\mathcal X = \mathcal Y = V_h \subset xxxxx$ is a finite element space (FEM) with a certain mesh. Typically, let us consider $\Omega = [0,1]^2$ and $\mathcal X = \mathcal Y$ as the linear finite element space with uniform mesh and $\frac{1}{d}$ mesh size. That is, 
$
    \mathcal X = \mathcal Y \cong \mathbb R^{d\times d}.
$
As a result, 
$
    \mathcal L (\mathcal X, \mathcal Y) = \mathcal L(\mathcal Y, \mathcal Y) \cong \mathbb R^{d^2 \times d^2},
$
which is too large to parametrize naively and directly. Hence, we resort to the well-acknowledge multigrid algorithm which have been applied solving many PDEs. Multigrid can be viewed as a linear operator between finite-dimensional function spaces. The algorithm identify the operator within $\mathcal{O}(\log N)$ parameters and $\mathcal{O}(N \log N)$ computational costs.  In particular, we consider the following linear V-cycle multigrid algorithm.  Our neural operator architecture is aligned with the linear V-cycle multigrid algorithm via translating the multigrid algorithm into a neural network.

\paragraph{How to parameterize $\mathcal B^\ell$}
It is important to parameterize $\mathcal B^\ell \in \mathcal Y^{n_\ell}$ efficiently.
even if $\mathcal X = \mathcal Y$ are finite-dimensional spaces, ...
Essentially, it is equivalent to parameterizing (discretizing) the space $\mathcal Y$. In particular, one may find a basis 
\begin{equation}
    \left\{y^\ell_0, y^\ell_1, \cdots, y^\ell_{m_\ell}\right\} \subset \mathcal Y
\end{equation}
and then parametrize $\mathcal B^\ell_i$ as
\begin{equation}
    \mathcal B^\ell_i = \sum_{j=0}^{m_\ell}  b^\ell_{ij} y^\ell_j,
\end{equation}
where $b^\ell_{ij} \in \mathbb R$.
As shown in the proof of the universal approximation properties for shallow neural operators, it is enough to parameterize
\begin{equation}
    \mathcal B^\ell_i = b^\ell_i \bm y_\sigma \in \mathcal Y.
\end{equation}
As we mentioned before, for the point-wise activation operator, we have $\bm y_\sigma = \bm 1(x)$.
That is, we can choose $y^\ell_0 = \bm 1(x)$ as the basis of constant functions.
Additionally, given that $\bm h^{\ell-1}_i \in \mathcal Y$ for all $i=1:n_{\ell-1}$, the following set
\begin{equation}
    \left\{\bm h^{\ell-1}_1, \cdots, \bm h^{\ell-1}_{n_{\ell-1}}\right\} \subset \mathcal Y
\end{equation}
forms a natural ``basis'' of $\mathcal Y$. That is, we may take $m_\ell = n_{\ell-1}$ and 
\begin{equation}
    y^\ell_i = \bm h^{\ell-1}_i.
\end{equation}
By combining these two parts together, we have
\begin{equation}
    \mathcal B^\ell_i = \sum_{j=1}^{n_{\ell-1}} b^\ell_{ij} \bm h^{\ell-1}_j + b^\ell_{i0} \bm 1(x).
\end{equation}
In the vector form, it can be expressed as
$
    \mathcal B^\ell =  \bm B^\ell \bm h^{\ell-1} + b^\ell
$
where
$
\bm B^\ell \in \mathbb R^{n_\ell\times n_{\ell-1}}, \quad \text{and} \quad b^\ell \in \mathbb R^{n_\ell}.
$

\begin{theorem}[informal]
	If $a(x)$ and $f(x)$ are smooth, then there exists $\Phi_\theta(a_h, f_h; u_h^0)$ such that
	$u_h = \Phi_\theta(a_h, f_h; u_h^0)$ can recover the solution of one-step V-cycle with Richardson iteration smoother for discrete system by linear finite element.
\end{theorem}
Some numerical tests to try:
\begin{itemize}
	\item more channels;
	\item how to define $f^{\ell+1}$;
	\item same questions to $a^{\ell+1}$;
	\item how to choose $B^{\ell,i}$, $\widetilde B^{\ell,i}$;
        \item change $B^{\ell,i}\ast$ to $B^{\ell,i}\tilde \ast$
	\item how to choose $\widetilde K^\ell$;
	\item ...
\end{itemize}

\subsection{MgNet on image segmentation}
Start from the 
\begin{equation}
    -\operatorname{div}(a \nabla u) + \delta u(1-u)^2 =f 
\end{equation}
to develop a MgNet variant to do image segmentation.

\section{Generalization error in large data regime}


\subsection{FDM scheme (fast example for verification)}
Then, it is equivalent to 
\begin{equation}\label{key}
	\begin{cases}
		- \left(a \Delta u + \nabla a \nabla u\right) = f, \quad &\text{in } \Omega, \\
		u = 0, \quad &\text{on } \partial \Omega.
	\end{cases}
\end{equation}
By using the central difference scheme, we have
\begin{equation}
-\left(a_{i,j} [K_{\Delta}\ast u]_{i,j} + [K_x\ast a]_{i,j}[K_x\ast u]_{i,j} + [K_y\ast a]_{i,j}[K_y\ast u]_{i,j} \right) = f_{i,j}
\end{equation}
This can be further reduced to
\begin{equation}
- \left(a \Delta u + \nabla a \nabla u\right) \approx [K_{i,j}\ast u]_{i,j} = f_{i,j}
\end{equation}
where
\begin{equation}
    K_{i,j} = a_{i,j} K_{\Delta} + [K_x\ast a]_{i,j} K_x + [K_y\ast a]_{i,j} K_y.
\end{equation}

==> MgNet2.tex <==
\section{MgNet without training for operator learning}
In this section, we propose to build a MgNet-based CNN architecture to solve
\begin{equation}\label{eq:PDE}
	\begin{cases}
		- \nabla \cdot \left(a(x) \nabla u\right) = f, \quad &\text{in } \Omega, \\
		u = 0, \quad &\text{on } \partial \Omega,
	\end{cases}
\end{equation}
where $\Omega = (0,1)^2$. Here, we consider approximating the following iterative operator
\begin{equation}\label{key}
	u \leftarrow \Phi_\theta(a,f; u),
\end{equation}
by MgNet. In particular, we will construct $ \Phi_\theta$ based on MgNet to solve the discretized \eqref{eq:PDE} as
\begin{equation}\label{key}
	u_h \approx u_h^k = \Phi_\theta(a_h,f_h; u_h^{k-1}),
\end{equation}
where $a_h, f_h, u_h \in \mathbb{R}^{n_1 \times m_1}$ and $u_h^0 = 0 \in \mathbb{R}^{n_1 \times m_1}$ or random by default. Then, we have the following network architecture.
\begin{algorithm}[H]
	\footnotesize
	\caption{$u  = \Phi_\theta(a_h, f_h; u_h^0)$}
	\label{alg:mgnet}
	\begin{algorithmic}[1]
		\STATE {\bf Input}: number of grids J, number of smoothing iterations $\nu_\ell$ for $\ell=1:J$, 
		number of channels $c_{f,\ell}$ for $f^\ell$ and $c_{u,\ell}$ for $u^{\ell,i}$ on $\ell$-th grid.
		\STATE Initialization:  $a^1 = a_h$, $f^1 = f_h$, $u^{1,0}=u_h^0$
		%		\STATE Initialization $u^{1,0}$
		\FOR{$\ell = 1:J$}
		\FOR{$i = 1:\nu_\ell$}
		\STATE Pre-smoothing:
		\begin{equation}\label{eq:mgnet}
			u^{\ell,i} = u^{\ell,i-1} +  B^{\ell,i} \widetilde \ast \left({f^\ell - A(a^\ell) \widetilde \ast u^{\ell,i-1}}\right) \in \mathbb{R}^{c_{u,\ell}\times n_\ell\times m_\ell}.
		\end{equation}
		\ENDFOR
		\STATE Note: 
		$
		u^\ell= u^{\ell,\nu_\ell} 
		$
		\STATE Interpolation and restriction:
		\begin{align}
			\label{eq:interpolation}
			u^{\ell+1,0} &= \Pi_\ell^{\ell+1}\ast_2u^{\ell} \in \mathbb{R}^{c_{u,\ell+1}\times n_{\ell+1}\times m_{\ell+1}} \\
                \label{eq:restrict-a}
			a^{\ell+1} &= C \ast_2 a^\ell \\
			\label{eq:restrict-f}
			f^{\ell+1} &= R^{\ell+1}_\ell \ast_2 \left(f^\ell - A(a^\ell) \widetilde \ast u^{\ell}\right) + A(a^{\ell+1}) \widetilde \ast u^{\ell+1,0}
			\end{align}
		\ENDFOR
		\FOR{$\ell = J-1:1$}
		\STATE Prolongation:
		\begin{equation}\label{key}
			u^{\ell,0} = u^{\ell} + \Pi_{\ell+1}^{\ell}\ast^2(u^{\ell+1} - u^{\ell+1,0})
		\end{equation}
		\FOR{$i = 1:\nu_\ell$}
		\STATE Post-smoothing:
		\begin{equation}\label{eq:mgnet}
			u^{\ell,i} = u^{\ell,i-1} + \widetilde B^{\ell,i} \widetilde \ast \left({f^\ell - A(a^{\ell}) \widetilde \ast u^{\ell,i-1}}\right) \in \mathbb{R}^{c_{u,\ell}\times n_\ell\times m_\ell}.
		\end{equation}
		\ENDFOR
		\ENDFOR
        \STATE {\bf Output:} $u = u^{1,\nu_1}$
	\end{algorithmic}
\end{algorithm}


Here, we notice that $\Phi_\theta(a_h, f_h; u_h^0)$ is a linear function in terms of $f_h$ and $u_h^0$ while it is a non-linear function (special polynomial) with respect to $a_h$.
Firstly, a crucial construction is to represent $a^\ell$ with two channels. Based on this representation, we have the following two main features in our work:
\begin{itemize}
    \item Generating the kernel $A(a^\ell)$ by using a fixed convolution kernel $K$;
    \item Finding the connection between $a^{\ell+1}$ and $e^\ell$ with a pure convolutional structure.
\end{itemize}
In addition, $A(a^\ell) \widetilde \ast u^{\ell}$ is another key feature in this architecture, where 
$A(a^\ell)  \in \mathbb{R}^{5 \times n_\ell \times m_\ell}$ and $A(a^\ell) \widetilde \ast u^{\ell}$ means the convolution with different $3\times 3$ (only five non-zero components) kernel on each grid point of $u^\ell$. More


\subsection{Commutative graph for efficiently constructing $A_{2h}$}

Here, we hope to find the projection from $a_h$ to $a_{2h}$ by using convolutional operators to get the following commutative graph for efficiently constructing $A_{2h}$.
\begin{equation}
\begin{tikzcd}
  a_h \arrow[r, "K\ast"] \arrow[d, red, "C\ast_2" red]
    & A_h \arrow[d, "P_{2h}^{h}", "R_{h}^{2h}"'] \\
  a_{2h} \arrow[r, "K\ast"]
&  A_{2h} 
\end{tikzcd}
\end{equation}

Firstly, we define $a_h$ as 
\begin{equation}
    \int_{K_i} a(x) dx.
\end{equation}
The main trick is to introduce an extra channel to denote $K_i$ such that each channel has a uniform dimension. It can be demonstrated as follows.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\textwidth]{TwoChannelK.png}
\end{figure}
As a result, we define
\begin{equation}
    a_h \in \mathbb R^{2\times n \times n}
\end{equation}
as
\begin{equation}
    [a_h]_{cij} = \int_{K_{cij}}a(x)dx
\end{equation}
for any $c=1:2$ and $i,j=1:n$.
Now, we show how to form $a_{2h}$ by using $a_h$. The coarse mesh is also demonstrated as follows.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\textwidth]{KtoKc.png}
\end{figure}

The following construction is the key.
\begin{equation}
\begin{aligned}
    [a_{2h}]_1 &= \begin{pmatrix}
        1 & 1 \\ 1 & 0
    \end{pmatrix} \ast_2 [a_h]_1 + \begin{pmatrix}
        1 & 0 \\ 0 & 0
    \end{pmatrix}\ast_2 [a_h]_2 \\
    [a_{2h}]_2 &= \begin{pmatrix}
        0 & 0 \\ 0 & 1
    \end{pmatrix} \ast_2 [a_h]_1 + \begin{pmatrix}
        0 & 1 \\ 1 & 1
    \end{pmatrix}\ast_2 [a_h]_2 
\end{aligned}
\end{equation}
Thus, we have
\begin{equation}
    a_{2h} = C\ast_2 a_h
\end{equation}
where
$C\in \mathbb R^{2\times 2\times 2\times 2}$ is a $2\times2$ kernel with two input channels and output channels.


\begin{proposition}
For P1 finite element discretization, there exists $K$ and $\phi$ such that, 
$$
A_h  u_h = (K *_1 a_h) \cdot (\phi *_1 u_h), 
$$ where $K \in \mathbb{R}^{2
\times 5 \times 3 \times 3}$ is $3\times3$ kernel with 2 input channel  and 5 output channel, $K*_1 a_h \in \mathbb{R}^{5\times (n-1) \times (n-1)}$ and $\phi \in \mathbb{R}^{5
\times 1 \times 3 \times 3}$, $\phi*u_h \in \mathbb{R}^{5\times (n-1) \times (n-1)}$,  $\cdot$ is pointwise inner product.  Similarly  
$$
A_{2h}  u_{2h} = (K *_1 a_{2h}) \cdot (\phi *_1 u_{2h}). 
$$ 
However 
\end{proposition}

Now, we show the formulation of $K$ and $\phi$ and how to from $A_h\left(A_{2 h}\right)$ from $K$ and $\phi$.

We know  $[A u]_{i,j}$ is determined by the non-sharing kernel,
$$
A_{i j}=\left(\begin{array}{ccc}
0 & A^{0,1}_{i j} & 0 \\
A^{-1,0}_{i j} & A^{0,0}_{i j} & A^{1,0}_{i j} \\
0 & A^{0,-1}_{i j} & 0
\end{array}\right) = \sum A_{ij}^{p,q} \phi^{p,q}, 
$$
where $\phi^{0,1} = \left(\begin{array}{ccc}
0 & 1 & 0 \\
0 & 0 & 0 \\
0 & 0 & 0
\end{array}\right) $, $\phi^{0,-1} = \left(\begin{array}{ccc}
0 & 0 & 0 \\
0 & 0 & 0 \\
0 & 1 & 0
\end{array}\right)...$ form the basis of 3 by 3 kernel space. We let $\phi:=\left[ \phi^{0,0}, \phi^{0,1}, \phi^{0,-1}, \phi^{1,0}, \phi^{-1,0}\right] \in \mathbb{R}^{5\times1 \times3 \times 3}$. 
$$
\begin{aligned}
& A^{00}_{i j}=\left(\left[\begin{array}{ll}
0 & 1 \\
1 & 2
\end{array}\right] * a_1+\left[\begin{array}{ll}
2 & 1 \\
1 & 0
\end{array}\right] * a_2\right)_{i j} =  \left(\left[\left[\begin{array}{ll}
0 & 1 \\
1 & 2
\end{array}\right] , \left[\begin{array}{ll}
2 & 1 \\
1 & 0
\end{array}\right] \right]*   [a_1,a_2] \right)_{i j}\\
& A^{0,1}_{i j}=-\left(\left[\begin{array}{ll}
0 & 1 \\
0 & 0
\end{array}\right] * a_1+\left[\begin{array}{ll}
1 & 0 \\
0 & 0
\end{array}\right] * a_2\right)_{i j} \\
& A^{-1,0}_{i j}=-\left(\left[\begin{array}{ll}
0 & 0 \\
1 & 0
\end{array}\right] * a_1+\left[\begin{array}{ll}
1 & 0 \\
0 & 0
\end{array}\right] * a_2\right)_{i j} \\
& A_{0,-1}^{i j}=-\left(\left[\begin{array}{ll}
0 & 0 \\
0 & 1
\end{array}\right] * a_1+\left[\begin{array}{ll}
0 & 0 \\
1 & 0
\end{array}\right] * a_2\right)_{i j} \\
& A^{0,1}_{i j}=-\left(\left[\begin{array}{ll}
0 & 0 \\
0 & 1
\end{array}\right] * a_1+\left[\begin{array}{ll}
0 & 1 \\
0 & 0
\end{array}\right] * a_2\right)_{j j}
\end{aligned},
$$
Therefore, $K:= \left[ \left[\left[\begin{array}{ll}
0 & 1 \\
1 & 2
\end{array}\right] , \left[\begin{array}{ll}
2 & 1 \\
1 & 0
\end{array}\right] \right], \left[  -\left[\begin{array}{ll}
0 & 1 \\
0 & 0
\end{array}\right], -\left[\begin{array}{ll}
1 & 0 \\
0 & 0
\end{array}\right] \right], ... \right] $
\newcommand\myeq{\stackrel{\mathclap{\normalfont\mbox{ij}}}{\cdot}}


\subsection{Numerical details and results}

\begin{table}[H]
    \small
    \centering
    \begin{tabular}{c|cc}
    \hline
    Model & Evaluation time (ms) &  Relative $L^2$  error ($\times 10 ^{-2}$)  \\
    \hline
    FNO & \textbf{ 3 } & 0.78\\
    MgNet(FEM) & \textbf{ 0.7 } & 0.01\\
    MgNet(FEM) & \textbf{ 0.84 } & 0.0014\\
    MgNet(FEM) & \textbf{ 0.98 } & 0.0002\\
    MgNet(FEM) & \textbf{ 1.12 } & 4e-5\\
    \hline
    \end{tabular}
    \caption{Relative $L^2$ error and evaluation time on the Darcy rough benchmark. }
    \label{tab:evaluation runtime}
\end{table}
\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\textwidth]{fem_cov.png}
	\caption{Convergence in terms of iteration number}
\end{figure} 

==> old_materiel.tex <==
\section{Questions to consider}

\begin{itemize}
\item Is the linear nonlocal operator, $W\vh(\vx)+\vc+\mathcal{A}[\vh](\vx)$, a universal approximator to linear operators? If yes, what is the necessary and sufficient condition?
\item As stated in \citep{lanthaler2023nonlocal}, the neural operator $\gG$ is a universal approximator for any continuous operator $\Psi:C^s(\overline{\Omega};\mathbb R^{d_g})\rightarrow C^r(\overline{\Omega};\mathbb R^{d_u})$, $s,r\geq 0$, if we define $\gA$ as an averaging neural operators:
$$\kappa(\vx,\vy):=\dfrac{1}{|\Omega|},$$
and the key of the proof is to rewrite $\Psi$ as a linear combination of a function basis $\{\eta_1(\vx),\cdots,\eta_J(\vx)\}\subset C^r(\overline{\Omega};\mathbb R^{d_u})$:
\begin{equation}
\Psi[f]\approx\sum_{j=1}^J \alpha_j[f] \eta_j,
\end{equation}
where $\alpha_j:L^1(\Omega;\mathbb R^{d_g})\rightarrow \mathbb R$ are continuous functionals on $L^1$-functions.
\end{itemize}

\subsection{ MgNet approximation of $a \rightarrow u$ in Darcy flow}
Let  $f=1$ and we train the $\text{V-MgNet}(\cdot ; A(a;\Theta_1),\Theta_2)$ on  data pairs $\{(a_i, u_i)\}$, where $A(\cdot;\Theta_1)$ is a network maps the coefficient to kernels
\begin{lemma}
Let $\mathcal{U}=\left\{h \in L^{\infty}(\Omega),\, \exists h_0>0 \text { such that } h(x) \geq h_0 \text { in } \Omega\right\} .$
The map $h \mapsto u$ is continuous from $\mathcal{U}$ into $H_0^1(\Omega)$.
\end{lemma}
\begin{proof}
Let $h_n \in \mathcal{U}_{a d}$ be a sequence such that $\left\|h_n-h_{\infty}\right\|_{L^{\infty}(\Omega)} \rightarrow 0$. Let $u_n$ be the unique solution in $H_0^1(\Omega)$ of the membrane equation with the associated thickness $h_n$
$$
\begin{gathered}
\begin{cases}
-\operatorname{div}\left(h_n \nabla u_n\right)=f & \text { in } \Omega \\
u_n=0 & \text { on } \partial \Omega,\end{cases} \\
\Leftrightarrow \int_{\Omega} h_n \nabla u_n \cdot \nabla \phi d x=\int_{\Omega} f \phi d x \quad \forall \phi \in H_0^1(\Omega) .
\end{gathered}
$$
We substract the variational formulation for $u_m$ to that for $u_n$
$$
\int_{\Omega} h_n \nabla\left(u_n-u_m\right) \cdot \nabla \phi d x=\int_{\Omega}\left(h_m-h_n\right) \nabla u_m \cdot \nabla \phi d x \quad \forall \phi \in H_0^1(\Omega) .
$$
Choosing $\phi=u_n-u_m$ we deduce
$$
\left\|\nabla\left(u_n-u_m\right)\right\|_{L^2(\Omega)} \leq \frac{C}{h_{\min }^2}\|f\|_{L^2(\Omega)}\left\|h_m-h_n\right\|_{L^{\infty}(\Omega)},
$$
which proves that $u_n$ is a Cauchy sequence in $H_0^1(\Omega)$ and thus converges.
\end{proof}

\begin{lemma}
$$
\begin{cases}
-\operatorname{div}\left(h  \nabla u \right)=f & \text { in } \Omega \\
u =0 & \text { on } \partial \Omega,
\end{cases}
$$
The map $\mathcal{P}: h \mapsto u(h)$, which gives the solution $u(h) \in H_0^1(\Omega)$ for $h \in \mathcal{U}$, is differentiable and its directional derivative at $h$ in the direction $k \in L^{\infty}(\Omega)$ is given by
$$
\left\langle u^{\prime}(h), k\right\rangle=v, \quad 
$$
where $v$ is the unique solution in $H_0^1(\Omega)$ of
$$
\left\{\begin{array}{ll}
-\operatorname{div}(h \nabla v)=\operatorname{div}(k \nabla u) & \text { in } \Omega \\
v=0 & \text { on } \partial \Omega .
\end{array}\right.
$$
\end{lemma}

\begin{lemma}
For $h \in \mathcal{U}$, let $u(h)$ be the state in $H_0^1(\Omega)$ such that 
$$
\begin{cases}
-\operatorname{div}\left(h  \nabla u \right)=f & \text { in } \Omega \\
u =0 & \text { on } \partial \Omega,
\end{cases}
$$
and
$$
J(h):=\int_{\Omega} j(u(h)) d  x:=\int_{\Omega} u(h) \phi(x) d x.
$$ The functional $J(h): \mathcal{U} \rightarrow \mathbb{R}$, is differentiable and its directional derivative at $h$ in the direction $k \in L^{\infty}(\Omega)$ is given by
$$
\left\langle J^{\prime}(h), k\right\rangle=\int_{\Omega} \phi v d x,
$$
where $v=\left\langle u^{\prime}(h), k\right\rangle$ is the unique solution in $H_0^1(\Omega)$ of 
$$
\begin{cases}  
-\operatorname{div}(h \nabla v)=\operatorname{div}(k \nabla u) & \text { in } \Omega \\ v=0 & \text { on } \partial \Omega .\end{cases}
$$
We introduce an adjoint state $p$ defined as the unique solution in
$$
\begin{cases}
-\operatorname{div}(h \nabla p)=-j^{\prime}(u) = -\phi & \text { in } \Omega \\ p=0 & \text { on } \partial \Omega
\end{cases}
$$
Then the cost function $J(h)$ is differentiable on $\mathcal{U}$ and
$$
J^{\prime}(h)=\nabla u \cdot \nabla p,
$$
$$
\left\langle J^{\prime}(h), k\right\rangle = \int_{\Omega} k \nabla u \cdot \nabla p dx  ,
$$
\end{lemma}

\begin{remark}
    

    $\mathcal{F}(u) := \int_{\Omega} u(x) \phi(x) dx$. $\mathcal{U}=\left\{h \in L^{\infty}(\Omega),\, \exists h_0>0 \text { such that } h(x) \geq h_0 \text { in } \Omega\right\} .$ For $a \in \mathcal{U}$, let $u(a)$ be the state in $H_0^1(\Omega)$ such that 
$$
\begin{cases}
-\operatorname{div}\left(a  \nabla u \right)=f & \text { in } \Omega \\
u =0 & \text { on } \partial \Omega,
\end{cases}
$$
We define the functional 
    $$
    J(a ): = \mathcal{F}(u) , 
    $$
    Then the cost function $J(a)$ is differentiable on $\mathcal{U}$ and
$$
J^{\prime}(a; \xi)=\nabla u \cdot \nabla p,
$$
where the adjoint state $p$ satisfies the adjoint equation
$$
\begin{cases}
-\operatorname{div}(a \nabla p)= -\phi  & \text { in } \Omega \\ p=0 & \text { on } \partial \Omega
\end{cases}
$$
    % I suppose for larger $\xi$,  $\|J^{\prime}(a; \xi)\|$ is smaller,  and as such $J(a; \xi)$ is easier to generalize.

\end{remark}

\section{Model}
 The operator learning problem. Let $\mathcal{U}$ and $\mathcal{V}$ be two (possibly infinite-dimensional) separable Banach spaces with norm $\|\cdot\|_{\mathcal{U}}$, $\|\cdot\|_{\mathcal{V}}$ and suppose that
$$
\mathcal{G}^{\dagger}: \mathcal{U} \rightarrow \mathcal{V}
$$
is an arbitrary (possibly nonlinear) operator. Then, broadly speaking, the goal of operator learning is to approximate $\mathcal{G}^{\dagger}$ from a finite number $N$ of input/output data on $\mathcal{G}^{\dagger}$. For our framework, we consider the setting where the input/output data are only partially observed through a finite collection of linear measurements which we formalize as follows:




\subsection{Finite dimensional approximation}
\begin{assumption}
Let the interpolation operators be $\boldsymbol{\phi}^{*}: \mathbb{R}^N \rightarrow \mathcal{U} $ and $\boldsymbol{\varphi}^*: \mathbb{R}^N\rightarrow  \mathcal{V}$. Assume for any $u \in \mathcal{U}$ and $v \in \mathcal{V}$, there exist $\boldsymbol{\phi}^{*}$, $\boldsymbol{\varphi}^*$ and $C$ such that
\begin{equation}
\begin{aligned}
      \|u-\boldsymbol{\phi}^{*}\boldsymbol{\phi} u\| \leq C d_N(\mathcal{U}) \\
      \|v-\boldsymbol{\varphi}^{*}\boldsymbol{\varphi} v\| \leq C d_N(\mathcal{V})
\end{aligned} 
\end{equation}
where $C$ is independent of $N$ and the Kolmogorov $N$-width is defined as
$$
d_N(\mathcal{U}):=\inf _{\mathcal{U}_N \subset \mathcal{U} ; \operatorname{dim} \mathcal{U}_N=N} \sup _{u \in \mathcal{U}} \inf _{u_N \in \mathcal{U}_N}\left\|u-u_N\right\|,
$$
\end{assumption}

\begin{remark}[Numerical homogenization]
Let $\mathcal{L}:=-div(a \nabla \cdot)$, where $a \in L^{\infty}(\Omega)$ is elliptic coefficient,
\begin{equation}
\mathcal{V}:=\{ v | \, \mathcal{L} v \in L^2(\Omega),   v =0 \text{ on } \partial \Omega \}.
\end{equation}
Let $\phi_i\in \mathcal{V}'$ be volume average functional  for $\tau_i\in \mathcal{T}$, such that 
$\left<\phi_i, v\right>:=1/|\tau_i|\int_{\tau_i} v d x$, then the interpolation operator can be defined as
$$
\boldsymbol{\phi}^*= (\mathcal{L}^{-1}\boldsymbol{\phi})(\vphi^T \mathcal{L}^{-1} \vphi)^{-1}
$$      
\end{remark}

\begin{remark}[Kernel regression]
As a prototypical example, consider the $\mathcal{U}$  are endowed with an RKHS structure induced with a kernel $Q: \Omega \times \Omega \rightarrow \mathbb{R}$.  We use kernel/GP regression to identify the maps $\vphi^*$.   



Let $\Omega$ be compact set with Lipschitz boundary, $X=\left(X_1, \ldots, X_n\right) \subset \Omega$   be distinct collections of points and define their fill-distances
$$
h_X:=\max _{x^{\prime} \in \Omega} \min _{x \in X}\left|x-x^{\prime}\right|, 
$$
In the case, we let $\left<\phi_i, u\right>:= u(X_i)$.
$\vphi^*$   can be expressed in closed form using standard representer theorems for kernel interpolation:
 $\vphi^*(U)(x)=Q(x, X) Q(X, X)^{-1} U,$
where $Q(X, X)$ is kernel matrices with entries $Q(X, X)_{i j}=Q\left(X_i, X_j\right)$  while $Q(x, X)$ and  denote row-vector fields with entries $Q(x, X)_i=Q\left(x, X_i\right)$.
\citep{arcangeli2007extension}
\begin{theorem}
    Suppose $Q$ is chosen such that $\mathcal{U}$ is continuously embedded in $H^t$ with $t > d_{\Omega}/2$. Then we have
    \begin{equation}
        \|u-\vphi^* \vphi(u)\|_{H^s(\Omega)} \lesssim h_X^{t-s}\|u-\vphi^* \vphi(u)\|_Q 
    \end{equation}
    \begin{proof}
        Since $(u-\vphi^*  \vphi(u))(X)=0$, using the sampling inequality for interpolation in Sobolev spaces \citep[Thm. 4.1]{arcangeli2007extension}, there exists a constant $h_{\Omega}>0$ so that if $h_X<h_{\Omega}$ then
 $\|u-\vphi^* \vphi(u)\|_{H^{s}(\Omega)} \leq C_{\Omega}^{\prime} h_X^{t-s}\|u-\vphi^*  \vphi(u)\|_{H^s(\Omega)} \leq C_{\Omega} h_X^{t-s}\|u-\vphi^* \vphi(u)\|_Q$,
where $C_{\Omega}^{\prime}, C_{\Omega}>0$ are constants that are independent of $u$. Using $\|u-\vphi^*  \vphi(u)\|_Q \leq\|u\|_Q$ and  $[2$, Thm. 12.3] we deduce the desired bound.
\end{proof}
\end{theorem}
\end{remark}

\begin{theorem}

    Consider the $\mathcal{U}$  are endowed with an RKHS structure induced with a kernel $Q: \Omega \times \Omega \rightarrow \mathbb{R}$.  Let $\Omega$ be compact set with Lipschitz boundary. 
 $X=\left(X_1, \ldots, X_N\right) \subset \Omega$   be distinct collections of points and define their fill-distances
$$
h_X:=\max _{x^{\prime} \in \Omega} \min _{x \in X}\left|x-x^{\prime}\right|, 
$$
The kernel interpolation 
$\hat{u}(x):= Q(x, X) Q(X, X)^{-1} U,$ where $U$ is a vector with $U_i = u(X_i)$,  $Q(X, X)$ is kernel matrices with entries $Q(X, X)_{i j}=Q\left(X_i, X_j\right)$  while $Q(x, X)$ and  denote row-vector fields with entries $Q(x, X)_i=Q\left(x, X_i\right)$. 

Suppose $Q$ is chosen such that $\mathcal{U}$ is continuously embedded in $H^t$ with $t > d/2$. Then we have
    \begin{equation}
        \|u-\vphi^* \vphi(u)\|_{H^s(\Omega)} \lesssim N^{\frac{t-s}{d}}\|u-\vphi^* \vphi(u)\|_Q 
    \end{equation}
\end{theorem}




In the case, we let $\left<\phi_i, u\right>:= u(X_i)$.
$\vphi^*$   can be expressed in closed form using standard representer theorems for kernel interpolation:
 $\vphi^*(U)(x)=Q(x, X) Q(X, X)^{-1} U,$
where $Q(X, X)$ is kernel matrices with entries $Q(X, X)_{i j}=Q\left(X_i, X_j\right)$  while $Q(x, X)$ and  denote row-vector fields with entries $Q(x, X)_i=Q\left(x, X_i\right)$.
\citep{arcangeli2007extension}
\begin{theorem}
    Suppose $Q$ is chosen such that $\mathcal{U}$ is continuously embedded in $H^t$ with $t > d_{\Omega}/2$. Then we have
    \begin{equation}
        \|u-\vphi^* \vphi(u)\|_{H^s(\Omega)} \lesssim h_X^{t-s}\|u-\vphi^* \vphi(u)\|_Q 
    \end{equation}
    \begin{proof}
        Since $(u-\vphi^*  \vphi(u))(X)=0$, using the sampling inequality for interpolation in Sobolev spaces \citep[Thm. 4.1]{arcangeli2007extension}, there exists a constant $h_{\Omega}>0$ so that if $h_X<h_{\Omega}$ then
 $\|u-\vphi^* \vphi(u)\|_{H^{s}(\Omega)} \leq C_{\Omega}^{\prime} h_X^{t-s}\|u-\vphi^*  \vphi(u)\|_{H^s(\Omega)} \leq C_{\Omega} h_X^{t-s}\|u-\vphi^* \vphi(u)\|_Q$,
where $C_{\Omega}^{\prime}, C_{\Omega}>0$ are constants that are independent of $u$. Using $\|u-\vphi^*  \vphi(u)\|_Q \leq\|u\|_Q$ and  $[2$, Thm. 12.3] we deduce the desired bound.
\end{proof}
\end{theorem}
 

\subsection{Modeling error}
\begin{itemize}
    \item Step 1: Analysis the error $\|\mathcal{G}^{\dagger} -\vvarphi^* 
    \mG \vphi\|$, where 
    $\mG :\mathbb{R}^N \rightarrow \mathbb{R}^N$ is defined by 
    $\mG(U):=\vvarphi \mathcal{G}^{\dagger}\vphi^*(U)$.
    \item Step 2: Approximate $\mG$ by neural network $\mG^{n}:\mathbb{R}^N \rightarrow \mathbb{R}^N$.
\end{itemize}
Next, we analysis the second step.

\begin{theorem}
Assume that  $\mathcal{G}^{\dagger}$ is a continuous operator such that 
\begin{equation}
    \|\rG u- \rG u'\|_{\mathcal{V}} \leq \ell (\|u-u'\|_{\mathcal{U}})
    \label{eqn:contin}
\end{equation}
and $u,u' \in \mathcal{K}$, where $\mathcal{K}$ is a compact subset of $\mathcal{U}$. Then we have
\begin{equation}
    \left\|\mathcal{G}^{\dagger}(u)- \vvarphi^* \mG \vphi(u) \right\|_{\mathcal{V}}   \leq C(\ell(d_N(\mathcal{K})) + d_N(\rG(\mathcal{K})))
\end{equation}

\begin{proof}
    By the definition of $\mG$ and the triangle inequality we have
$$
\begin{aligned}
\left\|\mathcal{G}^{\dagger}(u)- \vvarphi^* \vvarphi \mathcal{G}^{\dagger}\vphi^*\vphi(u) \right\|_{\mathcal{V}} \leq & \left\|\mathcal{G}^{\dagger}(u)-\mathcal{G}^{\dagger}   \vphi^*  \vphi(u)\right\|_{\mathcal{V}} \\
& +\left\|\mathcal{G}^{\dagger}  \vphi^*  \vphi(u)- \vvarphi^* \vvarphi  \mathcal{G}^{\dagger}  \vphi^*\vphi(u)\right\|_{\mathcal{V}} 
\end{aligned}
$$
Applying the continuous property \eqref{eqn:contin}, it yields 
$$
\begin{aligned}
\left\|\mathcal{G}^{\dagger}(u)-\mathcal{G}^{\dagger}   \vphi^*  \vphi(u)\right\|_{\mathcal{V}} \leq & \ell (\|u - \vphi^*  \vphi(u)\|) \leq C\ell(d_N(\mathcal{K}))  \\
\left\|\mathcal{G}^{\dagger}  \vphi^*  \vphi(u)- \vvarphi^* \vvarphi  \mathcal{G}^{\dagger}  \vphi^*  \vphi(u)\right\|_{\mathcal{V}}  \leq & C d_N(\rG(\mathcal{K}))
\end{aligned}
$$
\end{proof}
\begin{remark}
    From the above remarks, it is reasonable to expect the $ d_N(\rG(\mathcal{K})$ and $ d_N(\rG(\mathcal{K})  \sim \mathcal{O}(N^{-l(s,d)})$, where $l(s,d)$ is function depending on  regularity  $s$ and dimension $d$. 
\end{remark}
\end{theorem}

Then, we analysis Step 2
\begin{lemma}
    For $k \geq 1$ write $D^k \mathcal{G}^{\dagger}$ for the functional derivative of $\mathcal{G}^{\dagger}$ of order $k$. Recall that for $u \in \mathcal{U}$, $D^k \mathcal{G}^{\dagger}(u)$ is a multilinear operator mapping $\otimes_{i=1}^k \mathcal{U}$ to $\mathcal{V}$. For $w_1, \ldots, w_k \in \mathcal{U}$ write $\left[D^k \mathcal{G}^{\dagger}(u), \otimes_{i=1}^k w_i\right]$ for the (multilinear) action of $D^k \mathcal{G}^{\dagger}(u)$ on $\otimes_{i=1}^k w_i$ and write $\left\|D^k \mathcal{G}^{\dagger}(u)\right\|$ for the smallest constant such that for $w_1, \ldots, w_k \in \mathcal{U}$
$$
\left\|\left[D^k \mathcal{G}^{\dagger}(u), \otimes_{i=1}^k w_i\right]\right\|_{\mathcal{V}} \leq\left\|D^k \mathcal{G}^{\dagger}(u)\right\| \prod_{i=1}^k\left\|w_i\right\|_{\mathcal{U}}
$$
Similarly, for $k \geq 1$ write $D^k \mG$ for the derivation tensor of $\mG$ of order $k$ (the gradient for $k=1$ and the Hessian for $k=2$, etc). Recall that for $U \in \mathbb{R}^n, D^k \mG(U)$ is a multilinear operator mapping $\otimes_{i=1}^k \mathbb{R}^n$ to $\mathbb{R}^n$. For $W_1, \ldots, W_k \in \mathbb{R}^n$ write $\left[D^k \mG(U), \otimes_{i=1}^k W_i\right]$ for the (multilinear) action of $D^k \mG(U)$ on $\otimes_{i=1}^k W_i$ and write $\left\|D^k \mG(U)\right\|$ for the smallest constant 
such that for $W_1, \ldots, W_k \in \mathbb{R}^n$
$$
\left|\left[D^k \mG(U), \otimes_{i=1}^k W_i\right]\right| \leq\left\|D^k \mG(U)\right\| \prod_{i=1}^k\left|W_i\right|
$$
where $|\cdot|$ is the Euclidean norm.
 
Then, it holds true that $\left\|D^k \mG(U)\right\| \leq\|\vvarphi\|\|\vphi^*\|^k\left\|D^k \mathcal{G}^{\dagger} \circ \vphi^*(U)\right\|, \forall U \in \mathbb{R}^n$.
\end{lemma}

\begin{proof}
The chain rule and the linearity of $\varphi$ and $\vphi^*$ imply that
$$
\left[D^k \mG(U), \otimes_{i=1}^k W_i\right]=\vvarphi\left[D^k \mathcal{G}^{\dagger} \circ \vphi^*(U), \otimes_{i=1}^k \vphi^*\left(W_i\right)\right]
$$
We then conclude the proof by writing
$$
\begin{aligned}
\left|\left[D^k \mG(U), \otimes_{i=1}^k W_i\right]\right| & \leq \|\vvarphi\|\left\|D^k \mathcal{G}^{\dagger}   (\vvarphi(U))\right\| \prod_{i=1}^k\left\|\vvarphi\left(W_i\right)\right\| \\
& \leq\|\vvarphi\|\|\vphi^*\|^k\left\|D^k \mathcal{G}^{\dagger}   \vphi^*(U)\right\| \prod_{i=1}^k\left|W_i\right|
\end{aligned}
$$
\end{proof}

\begin{lemma}[Siegel and Xu, 2020]
    Let $m \geq 0$ be an integer and $\Omega \subset \mathbb{R}^d$ a bounded domain. Then for any Schwartz function $v$, we have
$$
\|v\|_{H^m(\Omega)} \lesssim\|v\|_{B^m(\Omega)} \lesssim\|v\|_{H^{m+\frac{d}{2}+\epsilon}(\Omega)}
$$
\end{lemma}

\begin{lemma}[Siegel and Xu, 2020]
    Let $\Omega=[0,1]^d, 0 \leq s \leq m$, and $f \in B^m(\Omega)$. Then there is $M \lesssim\|f\|_{B^m(\Omega)}$ such that 
    \begin{equation}
        \inf _{f_n \in \Sigma_{n, M}}\left\|f-f_n\right\|_{H^s(\Omega)} \lesssim\|f\|_{B^m(\Omega)} n^{-\frac{1}{2}-\frac{m-s}{d}}
    \end{equation}
 
\end{lemma}

\begin{corollary}
Let $\mathcal{K}$ be a compact subset of $\mathcal{U}$, it suffices $\Bar{\mathcal{K}}:= \mathcal{K} \cup \vphi^*\vphi(\mathcal{K})$ is also a compact subset of $\mathcal{U}$.
Suppose 
$
\sup_{u\in \Bar{\mathcal{K}}} \left\|D^k \mathcal{G}^{\dagger}(u)\right\| \leq \infty, 
$ for $1\leq k \leq m+\frac{d}{2}+1$. Let  then we have
\begin{equation}
    \sup_{U\in  \vphi(\mathcal{K})}\left\|D^k \mG(U)\right\| \leq  \infty, \  \text{for }1\leq k \leq m+\frac{d}{2}+1,
\end{equation}
therefore, we have $\mG :\mathbb{R}^d\rightarrow \mathbb{R}^d $ is component-wisely in $B^{m}(\vphi(\mathcal{K}))$.
\end{corollary}

\begin{corollary}
    For each component $\mG_i:\mathbb{R}^d \rightarrow \mathbb{R}$, there exists $\mG^{(n)}_i \in \Sigma_{n, M}$ such that 
    \begin{equation}
         \left\|\mG_i-\mG^{(n)}_i\right\|_{C(\Omega)} \leq  \left\|\mG_i-\mG^{(n)}_i\right\|_{H^s(\Omega)} \lesssim\|\mG_i\|_{B^m(\Omega)} n^{-\frac{1}{2}-\frac{m-s}{d}}
    \end{equation}
    % Then, point-wisely we have for any $U\in \vphi(\mathcal{K})$,
    
    % \begin{equation}
    %     \left\|\mG_i(U)-\mG^{(n)}_i(U)\right\|_{2} \leq  \left\|\mG_i(U)-\mG^{(n)}_i(U)\right\|_{F} \left\|\mG_i-\mG^{(n)}_i\right\|_{H^s(\Omega)} \lesssim\|\mG_i\|_{B^m(\Omega)} n^{-\frac{1}{2}-\frac{m-s}{d}}
    % \end{equation}
\end{corollary}
